Composition and Control with Distilled Energy Diffusion Models and Sequential Monte Carlo

Diffusion models may be formulated as a time-indexed sequence of energy-based models, where the score corresponds to the negative gradient of an energy function. As opposed to learning the score directly, an energy parameterization is attractive as the energy itself can be used to control generation via Monte Carlo samplers. Architectural constraints and training instability in energy parameterized models have so far yielded inferior performance compared to directly approximating the score or denoiser. We address these deficiencies by introducing a novel training regime for the energy function through distillation of pre-trained diffusion models, resembling a Helmholtz decomposition of the score vector field. We further showcase the synergies between energy and score by casting the diffusion sampling procedure as a Feynman Kac model where sampling is controlled using potentials from the learnt energy functions. The Feynman Kac model formalism enables composition and low temperature sampling through sequential Monte Carlo.

==> plots/fractal_tree.tex <==
\begin{figure*}[b]
    \centering
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/ground_truth.png}
        \caption{Ground Truth}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_-0.05.png}
        \caption{$\gamma=-0.05$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_-0.04.png}
        \caption{$\gamma=-0.04$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_0.png}
        \caption{$\gamma=0.0$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_0.05.png}
        \caption{$\gamma=0.05$}
    \end{subfigure}% \
    \\
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_0.1.png}
        \caption{$\gamma=0.1$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_0.2.png}
        \caption{$\gamma=0.2$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_0.5.png}
        \caption{$\gamma=0.5$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_1.0.png}
        \caption{$\gamma=1.0$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{plots/fractal/fractal_plot_5.0.png}
        \caption{$\gamma=5.0$}
    \end{subfigure}%
    \caption{\textbf{SMC Sampling of Feynman Kac Diffusion Model} for $G(x_{t-1},x_t)=p(x_{t-1})^\gamma$ with different temperatures. The tree-shaped distribution, inspired by~\citet{karras2024guiding}, is obtained by fitting a Gaussian to each branch, and by stacking these Gaussian in a tree pattern.}   
    \label{fig:temp_tree}
\end{figure*}

==> sections/2.2_FKM.tex <==
\textbf{Feynman Kac Models.}
Just as in computational statistics, Sequential Monte Carlo (SMC) methods provide a promising alternative to MCMC without requiring one to run a Markov chain to convergence. In order to understand the full generality of how SMC enables a change of measure, we first describe the Feynman Kac model (FKM) framework \citep{chopin2020introduction}. A FKM consists of an initial distribution $M_0$; some time indexed Markov transition kernels $(M_t)_t$, which we can sample from; and non-negative potential functions $(G_t)_t$, $G_0: \mathcal{X} \rightarrow \mathbb{R}^+$, $G_t: \mathcal{X}^2 \rightarrow \mathbb{R}^+$. 
The use of potentials permits a change of measure from the proposal from Markov process \eqref{eq:proposal_measure} to the FKM distribution \eqref{eq:fk_measure}. This provides a great deal of flexibility for controlling generation.
\begin{align}
    &M(\mathrm{d}x_{0:T}) = M_0(\mathrm{d}x_0)\prod_{t=1}^{T}M_t(\mathrm{d}x_t|x_{t-1}) \label{eq:proposal_measure} \\ 
    &Q(\mathrm{d}x_{0:T}) \propto G_0(x_0)\prod_{s=1}^{T}G_s(x_s,x_{s-1})M(\mathrm{d}x_{0:T}) \label{eq:fk_measure} 
\end{align}
\textbf{SMC for Feynman Kac Models.}
The FKM \eqref{eq:fk_measure} can be approximately simulated with SMC or particle filtering. An SMC procedure entails propagating $N$ particles initially sampled from some distribution $M_0$ through a sequence of proposal; importance weighting and resampling steps. The resampling steps are crucial to ensuring computation is focused on promising particles, and to avoiding weight degeneracy.
 
\begin{algorithm}
        \caption{Generative SMC}
        \label{alg:pf}
        \setlength{\parindent}{0pt}
        \begin{algorithmic}
            \State{Sample $\bfX_{0}^{i}\stackrel{\text{i.i.d.}}{\sim} M_0$ ~for $i \in [N]$}
           \State{Weight $\omega_1^{i}=G_0(\bfX^{i}_0)$~for $i \in [N]$}
        \For{$t=1,...,T$}
            \State{Normalize weights $w^i_{t-1}\propto \omega^i_{t-1}$, $\sum_{i=1}^N  w^i_{t-1}=1$}
            \State{Resample $\tilde{\bfX}^i_{t-1}\sim \sum_{i=1}^N  w^i_{t-1} \delta_{\bfX^i_{t-1}}$ ~for $i \in [N]$}
                \State{Proposal $\bfX_{t}^{i}\sim M(\cdot|\tilde{\bfX}^i_{t-1})$  ~for $i \in [N]$}
                \State{Weight $\omega^i_t= G(\bfX_{t}^{i},\tilde{\bfX}^i_{t-1})$}
        \EndFor
        \State{{\bfseries Return:} samples $(\bfX_{T}^{i})_i$}
        \end{algorithmic}
        \end{algorithm}

\textbf{Guided}. Given conditioning signal $y$, a guided FKM uses proposal and potentials:
\begin{align}
    M_t(x_t|x_{t-1})&=q(x_t|x_{t-1},y) \\ G_t(x_t,x_{t-1}) &= \tfrac{p(y|x_{t})p(x_t|x_{t-1})}{q(x_t|x_{t-1},y)}
\end{align}

\textbf{Twisted}.
\begin{align}
    M_t(x_t|x_{t-1})&=q(x_t|x_{t-1},y) \\ G_t(x_t,x_{t-1}) &= \tfrac{p(y|x_{t})p(x_t|x_{t-1})}{p(y|x_{t-1})q(x_t|x_{t-1},y)}
\end{align}

==> sections/A2_checklist.tex <==
\newpage
\section*{Checklist}

% The checklist follows the references. For each question, choose your answer from the three possible options: Yes, No, Not Applicable.  
% You are encouraged to include a justification to your answer, either by referencing the appropriate section of your paper or providing a brief inline description (1-2 sentences). 
% Please do not modify the questions.  Note that the Checklist section does not count towards the page limit. Not including the checklist in the first submission won't result in desk rejection, although in such case we will ask you to upload it during the author response period and include it in camera ready (if accepted).

% In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.

\begin{enumerate}
    \item For all models and algorithms presented, check if you include:
    \begin{enumerate}
        \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. Yes.
        \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. Yes.
        \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. Not Applicable.
    \end{enumerate}
    \item For any theoretical claim, check if you include:
    \begin{enumerate}
        \item Statements of the full set of assumptions of all theoretical results. Yes.
        \item Complete proofs of all theoretical results. Yes.
        \item Clear explanations of any assumptions. Yes.
    \end{enumerate}

    \item For all figures and tables that present empirical results, check if you include:
    \begin{enumerate}
        \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). Yes.
        \item All the training details (e.g., data splits, hyperparameters, how they were chosen). Yes.
        \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). Yes.
        \item A description of the computing infrastructure used (e.g., type of GPUs, internal cluster, or cloud provider). Yes.
    \end{enumerate}

    \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
    \begin{enumerate}
        \item Citations of the creator if your work uses existing assets. Yes.
        \item The license information of the assets, if applicable. Yes.
        \item New assets either in the supplemental material or as a URL, if applicable. Yes.
        \item Information about consent from data providers/curators. Not Applicable.
        \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. Not Applicable.
    \end{enumerate}

    \item If you used crowdsourcing or conducted research with human subjects, check if you include:
    \begin{enumerate}
        \item The full text of instructions given to participants and screenshots. Not Applicable.
        \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. Not Applicable.
        \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. Not Applicable.
    \end{enumerate}
\end{enumerate}


==> tables/fid_afhq.tex <==
% \begin{table}[h]
% \caption{Sample Table Title} \label{sample-table}
% % \begin{center}
% % \addtolength{\tabcolsep}{-0.9mm}
% \begin{tabular}{lcc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{AFHQ-64}} \\
%  & NFE & FID  \\
% \cmidrule{2-3}
% \textbf{Diffusion Model} \\
% EDM  & $--$   & $2.35$     \\
% \cmidrule{2-3}
% \textbf{Flow Model} \\
% FM  & $100$   & $2.73$   \\
% \cmidrule{2-3}
% \textbf{Energy Parameterized} \\
% EDM (energy)  & $80$  & $8.91$   \\
% Ours          & $80$  & $4.75$   \\
% \end{tabular}
% % }
% % \end{center}
% \end{table}
\begin{table}[H]
\caption{} \label{sample-table}
\begin{center}
% \addtolength{\tabcolsep}{-0.9mm}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{AFHQ-64}} & \multicolumn{2}{c}{\textbf{FFHQ-64}} \\
 & NFE & FID  & NFE & FID  \\
\cmidrule{2-3} \cmidrule{4-5}
\textbf{Diffusion / Flow} \\
\begin{tabular}[c]{@{}l@{}}EDM  {\scriptsize \citet{karras2022elucidating}}\end{tabular} & $79$   & $2.35$  & $79$  & $2.61$     \\
\begin{tabular}[c]{@{}l@{}}FM {\scriptsize \citet{liu2022rectified}} \\ {\scriptsize \citet{lipman2022flow}}\end{tabular}  & $100$   & $2.73$ & $100$  & $3.30$  \\
\cmidrule{2-5}
\textbf{Energy} \\
EDM (energy)  & $79$  & $4.57$  & $79$  & $2.71$ \\
Ours          & $79$  & $3.88$  & $79$  & $2.64$ \\
\bottomrule
\end{tabular}
% }
\end{center}
\end{table}

==> tables/fid_celeba.tex <==
\begin{table}[h]
\caption{Sample Table Title} \label{sample-table}
% \begin{center}
% \addtolength{\tabcolsep}{-0.9mm}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{CELEBA-64}} \\
% \cmidrule(lr){1-2}
 & NFE & FID  \\
\cmidrule{2-3}
\textbf{Diffusion Model} \\
EDM  & $80$   & $1.89$     \\
% \cmidrule{2-3}
% \textbf{Flow Model} \\
% FM  & $--$   & $--$   \\
% MBFM  & $--$   &$--$   \\
\cmidrule{2-3}
\textbf{Energy Parameterized} \\
CD-LEBM  & $--$   & $37.87$  \\
ED-LEBM  & $--$   & $36.73$  \\
DAMC  & $--$   & $30.83$  \\
DRL  & $--$   & $5.98$  \\
EDM  & $80$   & $2.03$  \\
Ours          & $80$  & $1.95$   \\
\bottomrule
\end{tabular}
% }
% \end{center}
\end{table}

==> tables/fid_conditional_tab.tex <==
\begin{table}
  \caption{Frechet Inception Distance for conditional generative modelling}
  \label{sample-table}
  \centering
\begin{tabular}{llll}
                   Method                                     & Cifar10                   & CelebA & CelebaHQ (latent) \\ \hline
{Diffusion (EDM - re-implementation)} & {2.2}  & 3.12   & x                 \\
{Diffusion (conditional)} & {2.2}  & 3.12   & x                 \\
{Diffusion Energy Models (SMC)}            & {2.01} & x      & x     
{Diffusion Energy Models (MCMC conditional)}            & {2.01} & x      & x     \\
\end{tabular}
\end{table}
